Polynomial Complementation of Nondeterministic 2-Way Finite Automata by 1-Limited Automata

We prove that, paying a polynomial increase in size only, every unrestricted two-way nondeterministic finite automaton (2NFA) can be complemented by a 1-limited automaton (1-LA), a nondeterministic extension of 2NFAs still characterizing regular languages. The resulting machine is actually a restricted form of 1-LAs -- known as 2NFAs with common guess -- and is self-verifying. A corollary of our construction is that a single exponential is necessary and sufficient for complementing 1-LAs.

==> tikzlibrarygb-loops.code.tex <==
\RequirePackage{tikz}

% draw loops <<<
\tikzset{
	loop north/.style={in=75,out=105,loop},				%N
	loop north east/.style={in=15,out=45,loop},			%NE
	loop east/.style={in=345,out=15,loop},					%E
	loop south east/.style={in=-45,out=-15,loop},		%SE
	loop south/.style={in=255,out=285,loop},				%S
	loop south west/.style={in=255,out=225,loop},		%SW
	loop west/.style={in=165,out=195,loop},				%W
	loop north west/.style={in=165,out=135,loop},		%NW
	loop around/.style={in={#1-15},out={#1+15},loop}	%around angle
}

%parameters: "looseness" and "min distance"

